The ANU WiFeS SuperNovA Program (AWSNAP)

This paper presents the first major data release and survey description for the ANU WiFeS SuperNovA Program (AWSNAP). AWSNAP is an ongoing supernova spectroscopy campaign utilising the Wide Field Spectrograph (WiFeS) on the Australian National University (ANU) 2.3m telescope. The first and primary data release of this program (AWSNAP-DR1) releases 357 spectra of 175 unique objects collected over 82 equivalent full nights of observing from July 2012 to August 2015. These spectra have been made publicly available via the WISeREP supernova spectroscopy repository. We analyse the AWSNAP sample of Type Ia supernova spectra, including measurements of narrow sodium absorption features afforded by the high spectral resolution of the WiFeS instrument. In some cases we were able to use the integral-field nature of the WiFeS instrument to measure the rotation velocity of the SN host galaxy near the SN location in order to obtain precision sodium absorption velocities. We also present an extensive time series of SN 2012dn, including a near-nebular spectrum which both confirms its "super-Chandrasekhar" status and enables measurement of the sub-solar host metallicity at the SN site.

==> table_awsnap_spectra.tex <==
\begin{deluxetable}{lccr}
\tablewidth{0pt}
\tablecaption{All AWSNAP Spectra
\label{tab:all_awsnap_spectra}}
\tabletypesize{\small}
\tablehead{
%---------
\colhead{SN} & 
\colhead{Observation} & 
\colhead{Grating} & 
\colhead{Exposure} \\
\colhead{} & 
\colhead{Date} & 
\colhead{} & 
\colhead{Time (s)}
}
\startdata
\scriptsize
%------------------
SN~2009ip             &  2012-Oct-22  &  B3000  &   1200  \\
SN~2009ip             &  2012-Oct-22  &  R3000  &   1200  \\
SN~2009ip             &  2012-Oct-23  &  B7000  &   1200  \\
SN~2009ip             &  2012-Oct-23  &  R7000  &   1200  \\
SN~2009ip             &  2012-Sep-22  &  B3000  &   1200  \\
SN~2009ip             &  2012-Sep-22  &  R3000  &   1200  \\
SN~2009ip             &  2012-Sep-23  &  B3000  &   1200  \\
SN~2009ip             &  2012-Sep-23  &  R3000  &   1200  \\
SN~2009ip             &  2013-Apr-12  &  B7000  &   1200  \\
SN~2009ip             &  2013-Apr-12  &  R7000  &   1200  \\
SN~2009ip             &  2013-Jun-22  &  B7000  &   1200  \\
SN~2009ip             &  2013-Jun-22  &  R7000  &   1200  \\
SN~2009ip             &  2013-May-26  &  B3000  &   1200  \\
SN~2009ip             &  2013-May-26  &  R7000  &   1200  \\
SN~2012ca             &  2012-Aug-10  &  B3000  &   1200  \\
SN~2012ca             &  2012-Aug-10  &  R3000  &   1200  \\
SN~2012ca             &  2012-Sep-06  &  B3000  &   1200  \\
SN~2012ca             &  2012-Sep-06  &  R3000  &   1200  \\
SN~2012ca             &  2012-Sep-07  &  B3000  &   1200  \\
SN~2012ca             &  2012-Sep-07  &  R3000  &   1200  \\
SN~2012ca             &  2012-Sep-22  &  B3000  &   1200  \\
SN~2012ca             &  2012-Sep-22  &  R3000  &   1200  \\
SN~2012ca             &  2012-Sep-23  &  B3000  &   1200  \\
SN~2012ca             &  2012-Sep-23  &  R3000  &   1200  \\
SN~2012ca             &  2013-Jun-03  &  B3000  &   1200  \\
SN~2012ca             &  2013-Jun-03  &  R7000  &   1200  \\
SN~2012ca             &  2013-May-26  &  B3000  &   1200  \\
SN~2012ca             &  2013-May-26  &  R3000  &   1200  \\
SN~2012ca             &  2013-May-26  &  R7000  &   1200  \\
SN~2012dj             &  2012-Aug-11  &  B3000  &   1200  \\
SN~2012dj             &  2012-Aug-11  &  R3000  &   1200  \\
SN~2012dj             &  2012-Aug-12  &  B3000  &   1200  \\
SN~2012dj             &  2012-Aug-12  &  R3000  &   1200  \\
SN~2012dj             &  2012-Aug-13  &  B3000  &   1200  \\
SN~2012dj             &  2012-Aug-13  &  R3000  &   1200  \\
SN~2012dj             &  2012-Sep-06  &  B3000  &   1200  \\
SN~2012dj             &  2012-Sep-06  &  R3000  &   1200  \\
SN~2012dj             &  2012-Sep-07  &  B3000  &   1200  \\
SN~2012dj             &  2012-Sep-07  &  R3000  &   1200  \\
SN~2012dj             &  2012-Sep-22  &  B3000  &   1200  \\
SN~2012dj             &  2012-Sep-22  &  R3000  &   1200  \\
SN~2012dj             &  2012-Sep-23  &  B3000  &   1200  \\
SN~2012dj             &  2012-Sep-23  &  R3000  &   1200  \\
SN~2012dn             &  2012-Aug-11  &  B3000  &   1200  \\
SN~2012dn             &  2012-Aug-11  &  R3000  &   1200  \\
SN~2012dn             &  2012-Aug-12  &  B3000  &   1200  \\
SN~2012dn             &  2012-Aug-12  &  R3000  &   1200  \\
SN~2012dn             &  2012-Aug-13  &  B3000  &   1200  \\
SN~2012dn             &  2012-Aug-13  &  R3000  &   1200  \\
SN~2012dn             &  2012-Jul-18  &  B3000  &    600  \\
SN~2012dn             &  2012-Jul-18  &  R3000  &    600  \\
SN~2012dn             &  2012-Jul-19  &  B3000  &    600  \\
SN~2012dn             &  2012-Jul-19  &  R3000  &    600  \\
SN~2012dn             &  2012-Jul-20  &  B3000  &    180  \\
SN~2012dn             &  2012-Jul-20  &  R3000  &    180  \\
SN~2012dn             &  2012-Jul-21  &  B3000  &   1200  \\
SN~2012dn             &  2012-Jul-21  &  R3000  &   1200  \\
SN~2012dn             &  2012-Oct-23  &  B3000  &   1200  \\
SN~2012dn             &  2012-Oct-23  &  R3000  &   1200  \\
SN~2012dn             &  2012-Sep-06  &  B3000  &   1200  \\
SN~2012dn             &  2012-Sep-06  &  R3000  &   1200  \\
SN~2012dn             &  2012-Sep-07  &  B3000  &   1200  \\
SN~2012dn             &  2012-Sep-07  &  R3000  &   1200  \\
SN~2012dn             &  2012-Sep-22  &  B3000  &   1200  \\
SN~2012dn             &  2012-Sep-22  &  R3000  &   1200  \\
SN~2012dn             &  2012-Sep-23  &  B3000  &   1200  \\
SN~2012dn             &  2012-Sep-23  &  R3000  &   1200  \\
SN~2012dt             &  2012-Sep-22  &  B3000  &   1200  \\
SN~2012dt             &  2012-Sep-22  &  R3000  &   1200  \\
SN~2012dy             &  2012-Aug-11  &  B3000  &   1200  \\
SN~2012dy             &  2012-Aug-11  &  R3000  &   1200  \\
SN~2012dy             &  2012-Aug-12  &  B3000  &   1200  \\
SN~2012dy             &  2012-Aug-12  &  R3000  &   1200  \\
SN~2012dy             &  2012-Aug-13  &  B3000  &   1200  \\
SN~2012dy             &  2012-Aug-13  &  R3000  &   1200  \\
SN~2012dy             &  2012-Sep-06  &  B3000  &   1200  \\
SN~2012dy             &  2012-Sep-06  &  R3000  &   1200  \\
SN~2012dy             &  2012-Sep-07  &  B3000  &   1200  \\
SN~2012dy             &  2012-Sep-07  &  R3000  &   1200  \\
SN~2012dy             &  2012-Sep-22  &  B3000  &   1200  \\
SN~2012dy             &  2012-Sep-22  &  R3000  &   1200  \\
SN~2012dy             &  2012-Sep-23  &  B3000  &   1200  \\
SN~2012dy             &  2012-Sep-23  &  R3000  &   1200  \\
SN~2012ec             &  2012-Aug-12  &  B3000  &   1200  \\
SN~2012ec             &  2012-Aug-12  &  R3000  &   1200  \\
SN~2012ec             &  2012-Aug-13  &  B3000  &   1200  \\
SN~2012ec             &  2012-Aug-13  &  R3000  &   1200  \\
SN~2012ec             &  2012-Oct-22  &  B3000  &   1200  \\
SN~2012ec             &  2012-Oct-22  &  R3000  &   1200  \\
SN~2012ec             &  2012-Sep-01  &  B3000  &    600  \\
SN~2012ec             &  2012-Sep-01  &  R3000  &    600  \\
SN~2012ec             &  2012-Sep-03  &  B3000  &    700  \\
SN~2012ec             &  2012-Sep-03  &  R3000  &    700  \\
SN~2012ec             &  2012-Sep-06  &  B3000  &   1200  \\
SN~2012ec             &  2012-Sep-06  &  R3000  &   1200  \\
SN~2012ec             &  2012-Sep-07  &  B3000  &   1200  \\
SN~2012ec             &  2012-Sep-07  &  R3000  &   1200  \\
SN~2012ec             &  2012-Sep-22  &  B3000  &   1200  \\
SN~2012ec             &  2012-Sep-22  &  R3000  &   1200  \\
SN~2012ec             &  2012-Sep-23  &  B3000  &   1200  \\
SN~2012ec             &  2012-Sep-23  &  R3000  &   1200  \\
SN~2012eq             &  2012-Sep-07  &  B3000  &   1200  \\
SN~2012eq             &  2012-Sep-07  &  R3000  &   1200  \\
SN~2012eu             &  2012-Sep-07  &  B3000  &   1200  \\
SN~2012eu             &  2012-Sep-07  &  R3000  &   1200  \\
SN~2012hr             &  2013-Dec-30  &  B3000  &   1200  \\
SN~2012hr             &  2013-Dec-30  &  R3000  &   1200  \\
SN~2013K              &  2013-May-26  &  B3000  &   1200  \\
SN~2013K              &  2013-May-26  &  R3000  &   1200  \\
SN~2013aa             &  2013-Apr-09  &  B3000  &   1200  \\
SN~2013aa             &  2013-Apr-09  &  R3000  &   1200  \\
SN~2013aa             &  2013-Mar-25  &  B3000  &   1200  \\
SN~2013aa             &  2013-Mar-25  &  R3000  &   1200  \\
SN~2013aa             &  2013-Sep-13  &  B3000  &   1200  \\
SN~2013aa             &  2013-Sep-13  &  R3000  &   1200  \\
SN~2013aa             &  2014-Jan-31  &  B3000  &   1200  \\
SN~2013aa             &  2014-Jan-31  &  R3000  &   1200  \\
SN~2013ai             &  2013-Apr-09  &  B3000  &   1200  \\
SN~2013ai             &  2013-Apr-09  &  R3000  &   1200  \\
SN~2013ai             &  2013-Mar-08  &  B3000  &   1200  \\
SN~2013ai             &  2013-Mar-08  &  R3000  &   1200  \\
SN~2013ai             &  2013-Mar-25  &  B3000  &   1200  \\
SN~2013ai             &  2013-Mar-25  &  R3000  &   1200  \\
SN~2013ai             &  2013-May-26  &  B3000  &   1200  \\
SN~2013ai             &  2013-May-26  &  R3000  &   1200  \\
SN~2013aj             &  2013-Mar-08  &  B3000  &   1200  \\
SN~2013aj             &  2013-Mar-08  &  R3000  &   1200  \\
SN~2013aj             &  2013-Mar-25  &  B3000  &   1200  \\
SN~2013aj             &  2013-Mar-25  &  R3000  &   1200  \\
SN~2013am             &  2013-Apr-09  &  B3000  &   1200  \\
SN~2013am             &  2013-Apr-09  &  R3000  &   1200  \\
SN~2013am             &  2013-Mar-24  &  B3000  &   1200  \\
SN~2013am             &  2013-Mar-24  &  B3000  &   1800  \\
SN~2013am             &  2013-Mar-24  &  R3000  &   1200  \\
SN~2013am             &  2013-Mar-24  &  R3000  &   1800  \\
SN~2013am             &  2013-Mar-25  &  B3000  &   1200  \\
SN~2013am             &  2013-Mar-25  &  R3000  &   1200  \\
SN~2013am             &  2013-Mar-27  &  B3000  &   1500  \\
SN~2013am             &  2013-Mar-27  &  R3000  &   1500  \\
SN~2013ao             &  2013-Mar-25  &  B3000  &   1200  \\
SN~2013ao             &  2013-Mar-25  &  R3000  &   1200  \\
SN~2013bj             &  2013-Apr-12  &  B3000  &   1200  \\
SN~2013bj             &  2013-Apr-12  &  R3000  &   1200  \\
SN~2013bk             &  2013-Apr-12  &  B3000  &   1200  \\
SN~2013bk             &  2013-Apr-12  &  R3000  &   1200  \\
SN~2013by             &  2013-Aug-19  &  B3000  &   1200  \\
SN~2013by             &  2013-Aug-19  &  R3000  &   1200  \\
SN~2013by             &  2013-May-26  &  B3000  &   1200  \\
SN~2013by             &  2013-May-26  &  R3000  &   1200  \\
SN~2013by             &  2014-Jul-08  &  B3000  &   1200  \\
SN~2013by             &  2014-Jul-08  &  R3000  &   1200  \\
SN~2013bz             &  2013-May-26  &  B3000  &   1200  \\
SN~2013bz             &  2013-May-26  &  R3000  &   1200  \\
SN~2013cg             &  2013-May-26  &  B3000  &   1200  \\
SN~2013cg             &  2013-May-26  &  R3000  &   1200  \\
SN~2013cg             &  2013-May-26  &  R7000  &   1200  \\
SN~2013cs             &  2013-May-26  &  B3000  &   1200  \\
SN~2013cs             &  2013-May-26  &  R3000  &   1200  \\
SN~2013cs             &  2013-May-26  &  R7000  &   1200  \\
SN~2013cs             &  2014-Mar-22  &  B3000  &   1200  \\
SN~2013cs             &  2014-Mar-22  &  R3000  &   1200  \\
SN~2013cy             &  2013-Jun-03  &  B3000  &   1200  \\
SN~2013cy             &  2013-Jun-03  &  R3000  &   1200  \\
SN~2013cz             &  2013-Jun-03  &  B3000  &   1200  \\
SN~2013cz             &  2013-Jun-03  &  R3000  &   1200  \\
SN~2013df             &  2013-Jun-22  &  B3000  &   1200  \\
SN~2013df             &  2013-Jun-22  &  R3000  &   1200  \\
SN~2013dh             &  2013-Jul-01  &  B3000  &   1800  \\
SN~2013dh             &  2013-Jul-01  &  R3000  &   1800  \\
SN~2013dh             &  2013-Jun-22  &  B3000  &   1200  \\
SN~2013dh             &  2013-Jun-22  &  R3000  &   1200  \\
SN~2013du             &  2013-Jul-04  &  B3000  &   1200  \\
SN~2013du             &  2013-Jul-04  &  R3000  &   1200  \\
SN~2013ef             &  2013-Jul-04  &  B3000  &   1200  \\
SN~2013ef             &  2013-Jul-04  &  R3000  &   1200  \\
SN~2013ej             &  2013-Aug-11  &  B3000  &   1200  \\
SN~2013ej             &  2013-Aug-11  &  R3000  &   1200  \\
SN~2013ej             &  2013-Aug-19  &  B3000  &   1200  \\
SN~2013ej             &  2013-Aug-19  &  R3000  &   1200  \\
SN~2013ej             &  2013-Jul-31  &  B3000  &   1200  \\
SN~2013ej             &  2013-Jul-31  &  R3000  &   1200  \\
SN~2013ej             &  2013-Oct-16  &  B3000  &   1200  \\
SN~2013ej             &  2013-Oct-16  &  R3000  &   1200  \\
SN~2013ej             &  2013-Oct-24  &  B3000  &   1200  \\
SN~2013ej             &  2013-Oct-24  &  R3000  &   1200  \\
SN~2013ej             &  2013-Sep-19  &  B3000  &   1200  \\
SN~2013ej             &  2013-Sep-19  &  R3000  &   1200  \\
SN~2013ek             &  2013-Aug-11  &  B3000  &   1200  \\
SN~2013ek             &  2013-Aug-11  &  R3000  &   1200  \\
SN~2013ek             &  2013-Aug-19  &  B3000  &   1200  \\
SN~2013ek             &  2013-Aug-19  &  R3000  &   1200  \\
SN~2013ek             &  2013-Jul-31  &  B3000  &   1200  \\
SN~2013ek             &  2013-Jul-31  &  R3000  &   1200  \\
SN~2013ek             &  2013-Sep-13  &  B3000  &   1200  \\
SN~2013ek             &  2013-Sep-13  &  R3000  &   1200  \\
SN~2013er             &  2013-Jul-31  &  B3000  &   1200  \\
SN~2013er             &  2013-Jul-31  &  R3000  &   1200  \\
SN~2013fd             &  2013-Sep-19  &  B3000  &   1200  \\
SN~2013fd             &  2013-Sep-19  &  R3000  &   1200  \\
SN~2013fj             &  2013-Sep-19  &  B3000  &   1200  \\
SN~2013fj             &  2013-Sep-19  &  R3000  &   1200  \\
SN~2013fq             &  2013-Oct-24  &  B3000  &   1200  \\
SN~2013fq             &  2013-Oct-24  &  R3000  &   1200  \\
SN~2013fq             &  2013-Sep-19  &  B3000  &   1200  \\
SN~2013fq             &  2013-Sep-19  &  R3000  &   1200  \\
SN~2013fs             &  2013-Nov-14  &  B3000  &   1200  \\
SN~2013fs             &  2013-Nov-14  &  R3000  &   1200  \\
SN~2013fs             &  2013-Nov-28  &  B3000  &   1200  \\
SN~2013fs             &  2013-Nov-28  &  R3000  &   1200  \\
SN~2013fs             &  2013-Oct-08  &  B3000  &   1200  \\
SN~2013fs             &  2013-Oct-08  &  R3000  &   1200  \\
SN~2013fs             &  2013-Oct-24  &  B3000  &   1200  \\
SN~2013fs             &  2013-Oct-24  &  R3000  &   1200  \\
SN~2013ft             &  2013-Oct-08  &  B3000  &   1200  \\
SN~2013ft             &  2013-Oct-08  &  R3000  &   1200  \\
SN~2013fw             &  2013-Nov-14  &  B3000  &   1200  \\
SN~2013fw             &  2013-Nov-14  &  R3000  &   1200  \\
SN~2013gh             &  2013-Aug-19  &  B3000  &   1200  \\
SN~2013gh             &  2013-Aug-19  &  R7000  &   1200  \\
SN~2013gh             &  2013-Aug-30  &  B3000  &   1200  \\
SN~2013gh             &  2013-Aug-30  &  R3000  &   1200  \\
SN~2013gh             &  2013-Aug-30  &  R7000  &   1200  \\
SN~2013gi             &  2013-Nov-14  &  B3000  &   1200  \\
SN~2013gi             &  2013-Nov-14  &  R3000  &   1200  \\
SN~2013gq             &  2013-Oct-08  &  B3000  &   1200  \\
SN~2013gq             &  2013-Oct-08  &  R3000  &   1200  \\
SN~2013gr             &  2013-Dec-06  &  B3000  &   1200  \\
SN~2013gr             &  2013-Dec-06  &  R3000  &   1200  \\
SN~2013gr             &  2013-Dec-15  &  B3000  &   1200  \\
SN~2013gr             &  2013-Dec-15  &  R3000  &   1200  \\
SN~2013gr             &  2013-Dec-19  &  B3000  &   1200  \\
SN~2013gr             &  2013-Dec-19  &  R3000  &   1200  \\
SN~2013gr             &  2013-Dec-29  &  B3000  &   1200  \\
SN~2013gr             &  2013-Dec-29  &  R3000  &   1200  \\
SN~2013gr             &  2014-Jan-18  &  B3000  &   1200  \\
SN~2013gr             &  2014-Jan-18  &  R3000  &   1200  \\
SN~2013hh             &  2013-Dec-12  &  B3000  &   1200  \\
SN~2013hh             &  2013-Dec-12  &  R3000  &   1200  \\
SN~2013hj             &  2013-Dec-19  &  B3000  &   1200  \\
SN~2013hj             &  2013-Dec-19  &  R3000  &   1200  \\
SN~2013hj             &  2013-Dec-29  &  B3000  &   1200  \\
SN~2013hj             &  2013-Dec-29  &  R3000  &   1200  \\
SN~2013hn             &  2013-Dec-19  &  B3000  &   1200  \\
SN~2013hn             &  2013-Dec-19  &  R3000  &   1200  \\
SN~2013hn             &  2013-Dec-29  &  B3000  &   1200  \\
SN~2013hn             &  2013-Dec-29  &  R3000  &   1200  \\
SN~2013hn             &  2013-Jun-22  &  B3000  &   1200  \\
SN~2013hn             &  2013-Jun-22  &  R3000  &   1200  \\
SN~2013hu             &  2013-Dec-29  &  B3000  &   1200  \\
SN~2013hu             &  2013-Dec-29  &  R3000  &   1200  \\
SN~2013hx             &  2014-Feb-24  &  B3000  &   1200  \\
SN~2013hx             &  2014-Feb-24  &  R3000  &   1200  \\
SN~2013hx             &  2014-Jan-31  &  B3000  &   1200  \\
SN~2013hx             &  2014-Jan-31  &  R3000  &   1200  \\
SN~2013hx             &  2014-Mar-04  &  B3000  &   1200  \\
SN~2013hx             &  2014-Mar-04  &  R3000  &   1200  \\
SN~2013hx             &  2014-Mar-14  &  B3000  &   1200  \\
SN~2013hx             &  2014-Mar-14  &  R3000  &   1200  \\
SN~2014D              &  2014-Jan-18  &  B3000  &   1200  \\
SN~2014D              &  2014-Jan-18  &  R3000  &   1200  \\
SN~2014E              &  2014-Jan-18  &  B3000  &   1200  \\
SN~2014E              &  2014-Jan-18  &  R3000  &   1200  \\
SN~2014I              &  2014-Jan-18  &  B3000  &   1200  \\
SN~2014I              &  2014-Jan-18  &  R3000  &   1200  \\
SN~2014L              &  2014-Feb-24  &  B3000  &   1200  \\
SN~2014L              &  2014-Feb-24  &  R3000  &   1200  \\
SN~2014L              &  2014-Jan-31  &  B3000  &   1200  \\
SN~2014L              &  2014-Jan-31  &  R3000  &   1200  \\
SN~2014L              &  2014-Mar-14  &  B3000  &   1200  \\
SN~2014L              &  2014-Mar-14  &  R3000  &   1200  \\
SN~2014L              &  2014-Mar-22  &  B3000  &   1200  \\
SN~2014L              &  2014-Mar-22  &  R3000  &   1200  \\
SN~2014N              &  2014-Jan-31  &  B3000  &   1200  \\
SN~2014N              &  2014-Jan-31  &  R3000  &   1200  \\
SN~2014X              &  2014-Mar-04  &  B3000  &   1200  \\
SN~2014X              &  2014-Mar-04  &  R3000  &   1200  \\
SN~2014aa             &  2014-Apr-02  &  B3000  &   1200  \\
SN~2014aa             &  2014-Apr-02  &  R3000  &   1200  \\
SN~2014aa             &  2014-Mar-14  &  B3000  &   1200  \\
SN~2014aa             &  2014-Mar-14  &  R3000  &   1200  \\
SN~2014aa             &  2014-Mar-22  &  B3000  &   1200  \\
SN~2014aa             &  2014-Mar-22  &  R3000  &   1200  \\
SN~2014ac             &  2014-Mar-14  &  B3000  &   1200  \\
SN~2014ac             &  2014-Mar-14  &  R3000  &   1200  \\
SN~2014ad             &  2014-Apr-02  &  B3000  &   1200  \\
SN~2014ad             &  2014-Apr-02  &  R3000  &   1200  \\
SN~2014ad             &  2014-Apr-16  &  B3000  &   1800  \\
SN~2014ad             &  2014-Apr-16  &  R3000  &   1800  \\
SN~2014ad             &  2014-Apr-23  &  B3000  &   1200  \\
SN~2014ad             &  2014-Apr-23  &  R3000  &   1200  \\
SN~2014ad             &  2014-Mar-14  &  B3000  &   1200  \\
SN~2014ad             &  2014-Mar-14  &  R3000  &   1200  \\
SN~2014ad             &  2014-Mar-17  &  B3000  &   1800  \\
SN~2014ad             &  2014-Mar-17  &  R3000  &   1800  \\
SN~2014ad             &  2014-Mar-18  &  B3000  &   1800  \\
SN~2014ad             &  2014-Mar-18  &  R3000  &   1800  \\
SN~2014ad             &  2014-Mar-19  &  B3000  &   1800  \\
SN~2014ad             &  2014-Mar-19  &  R3000  &   1800  \\
SN~2014ad             &  2014-Mar-22  &  B3000  &   1200  \\
SN~2014ad             &  2014-Mar-22  &  R3000  &   1200  \\
SN~2014ad             &  2014-Mar-28  &  B3000  &   1000  \\
SN~2014ad             &  2014-Mar-28  &  R3000  &   1000  \\
SN~2014ah             &  2014-Apr-02  &  B3000  &   1200  \\
SN~2014ah             &  2014-Apr-02  &  R3000  &   1200  \\
SN~2014ao             &  2014-Apr-23  &  B3000  &   1200  \\
SN~2014ao             &  2014-Apr-23  &  R3000  &   1200  \\
SN~2014ao             &  2014-Apr-23  &  R7000  &   1200  \\
SN~2014ap             &  2014-Mar-22  &  B3000  &   1200  \\
SN~2014ap             &  2014-Mar-22  &  R3000  &   1200  \\
SN~2014at             &  2014-Apr-23  &  B3000  &   1200  \\
SN~2014at             &  2014-Apr-23  &  R3000  &   1200  \\
SN~2014at             &  2014-Apr-23  &  R7000  &   1200  \\
SN~2014au             &  2014-Apr-23  &  B3000  &   1200  \\
SN~2014au             &  2014-Apr-23  &  R3000  &   1200  \\
SN~2014bx             &  2014-Jul-22  &  B3000  &    200  \\
SN~2014bx             &  2014-Jul-22  &  R3000  &    200  \\
SN~2014bz             &  2014-Jun-11  &  B3000  &    800  \\
SN~2014bz             &  2014-Jun-11  &  R3000  &    800  \\
SN~2014ca             &  2014-Jun-11  &  B3000  &    800  \\
SN~2014ca             &  2014-Jun-11  &  R3000  &    800  \\
SN~2014cm             &  2014-Jun-11  &  B3000  &    800  \\
SN~2014cm             &  2014-Jun-11  &  R3000  &    800  \\
SN~2014co             &  2014-Jul-08  &  B3000  &   1200  \\
SN~2014co             &  2014-Jul-08  &  R3000  &   1200  \\
SN~2014cp             &  2014-Aug-05  &  B3000  &   1200  \\
SN~2014cp             &  2014-Aug-05  &  R3000  &   1200  \\
SN~2014cp             &  2014-Jul-08  &  B3000  &   1200  \\
SN~2014cp             &  2014-Jul-08  &  R3000  &   1200  \\
SN~2014cq             &  2014-Jul-08  &  B3000  &   1200  \\
SN~2014cq             &  2014-Jul-08  &  R3000  &   1200  \\
SN~2014cr             &  2014-Aug-05  &  B3000  &   1200  \\
SN~2014cr             &  2014-Aug-05  &  R3000  &   1200  \\
SN~2014cr             &  2014-Jul-08  &  B3000  &   1200  \\
SN~2014cr             &  2014-Jul-08  &  R3000  &   1200  \\
SN~2014cs             &  2014-Jul-08  &  B3000  &   1200  \\
SN~2014cs             &  2014-Jul-08  &  R3000  &   1200  \\
SN~2014ct             &  2014-Jun-12  &  B3000  &    800  \\
SN~2014ct             &  2014-Jun-12  &  R3000  &    800  \\
SN~2014cu             &  2014-Jul-08  &  B3000  &   1200  \\
SN~2014cu             &  2014-Jul-08  &  R3000  &   1200  \\
SN~2014cw             &  2014-Sep-09  &  B3000  &   1200  \\
SN~2014cw             &  2014-Sep-09  &  R3000  &   1200  \\
SN~2014cx             &  2014-Sep-09  &  B3000  &   1200  \\
SN~2014cx             &  2014-Sep-09  &  R3000  &   1200  \\
SN~2014cx             &  2014-Sep-10  &  B3000  &   1200  \\
SN~2014cx             &  2014-Sep-10  &  R3000  &   1200  \\
SN~2014cy             &  2014-Sep-09  &  B3000  &   1200  \\
SN~2014cy             &  2014-Sep-09  &  R3000  &   1200  \\
SN~2014dc             &  2014-Sep-10  &  B3000  &   1200  \\
SN~2014dc             &  2014-Sep-10  &  R3000  &   1200  \\
SN~2014df             &  2014-Jun-04  &  B3000  &    900  \\
SN~2014df             &  2014-Jun-04  &  R3000  &    900  \\
SN~2014dl             &  2014-Oct-03  &  B3000  &   1200  \\
SN~2014dl             &  2014-Oct-03  &  R3000  &   1200  \\
SN~2014dn             &  2014-Oct-03  &  B3000  &   1200  \\
SN~2014dn             &  2014-Oct-03  &  R3000  &   1200  \\
SN~2014dn             &  2014-Oct-09  &  B3000  &   1200  \\
SN~2014dn             &  2014-Oct-09  &  R3000  &   1200  \\
SN~2014do             &  2014-Oct-03  &  B3000  &   1200  \\
SN~2014do             &  2014-Oct-03  &  R3000  &   1200  \\
SN~2014dp             &  2014-Oct-09  &  B3000  &   1200  \\
SN~2014dp             &  2014-Oct-09  &  R3000  &   1200  \\
SN~2014dq             &  2014-Nov-14  &  B3000  &   1200  \\
SN~2014dq             &  2014-Nov-14  &  R3000  &   1200  \\
SN~2014dq             &  2014-Oct-27  &  B3000  &   1200  \\
SN~2014dq             &  2014-Oct-27  &  R3000  &   1200  \\
SN~2014dr             &  2014-Oct-18  &  B3000  &   1200  \\
SN~2014dr             &  2014-Oct-18  &  R3000  &   1200  \\
SN~2014eg             &  2015-Jan-29  &  B3000  &   1200  \\
SN~2014eg             &  2015-Jan-29  &  R7000  &   1200  \\
SN~2014eg             &  2015-Mar-05  &  B3000  &   1200  \\
SN~2014eg             &  2015-Mar-05  &  R3000  &   1200  \\
SN~2015F              &  2015-Apr-11  &  B3000  &   1200  \\
SN~2015F              &  2015-Apr-11  &  R3000  &   1200  \\
SN~2015F              &  2015-Apr-29  &  B3000  &   1200  \\
SN~2015F              &  2015-Apr-29  &  R3000  &   1200  \\
SN~2015F              &  2015-Jul-08  &  B3000  &   1200  \\
SN~2015F              &  2015-Jul-08  &  R3000  &   1200  \\
SN~2015F              &  2015-Mar-12  &  B3000  &   1200  \\
SN~2015F              &  2015-Mar-12  &  R3000  &   1200  \\
SN~2015J              &  2015-Aug-17  &  B3000  &   1200  \\
SN~2015J              &  2015-Aug-17  &  R7000  &   1200  \\
SN~2015J              &  2015-Jul-01  &  B3000  &   1200  \\
SN~2015J              &  2015-Jul-01  &  R7000  &   1200  \\
SN~2015J              &  2015-Jul-08  &  B3000  &   1200  \\
SN~2015J              &  2015-Jul-08  &  R7000  &   1200  \\
SN~2015J              &  2015-Jul-25  &  B3000  &    900  \\
SN~2015J              &  2015-Jul-25  &  R3000  &    900  \\
SN~2015J              &  2015-Jul-31  &  B3000  &   1200  \\
SN~2015J              &  2015-Jul-31  &  R3000  &   1200  \\
SN~2015J              &  2015-Jun-24  &  B3000  &   1200  \\
SN~2015J              &  2015-Jun-24  &  R3000  &   1200  \\
ASASSN-13co           &  2013-Sep-19  &  B3000  &   1200  \\
ASASSN-13co           &  2013-Sep-19  &  R3000  &   1200  \\
ASASSN-14dp           &  2014-Jul-08  &  B3000  &   1200  \\
ASASSN-14dp           &  2014-Jul-08  &  R3000  &   1200  \\
ASASSN-14eu           &  2014-Aug-05  &  B3000  &   1200  \\
ASASSN-14eu           &  2014-Aug-05  &  R3000  &   1200  \\
ASASSN-14ew           &  2014-Sep-10  &  B3000  &   1200  \\
ASASSN-14ew           &  2014-Sep-10  &  R3000  &   1200  \\
ASASSN-14fo           &  2014-Sep-10  &  B3000  &   1200  \\
ASASSN-14fo           &  2014-Sep-10  &  R3000  &   1200  \\
ASASSN-14fw           &  2014-Sep-10  &  B3000  &   1200  \\
ASASSN-14fw           &  2014-Sep-10  &  R3000  &   1200  \\
ASASSN-14gs           &  2014-Sep-09  &  B3000  &   1200  \\
ASASSN-14gs           &  2014-Sep-09  &  R3000  &   1200  \\
ASASSN-14ha           &  2014-Nov-06  &  B3000  &   1200  \\
ASASSN-14ha           &  2014-Nov-06  &  R3000  &   1200  \\
ASASSN-14ha           &  2014-Oct-03  &  B3000  &   1200  \\
ASASSN-14ha           &  2014-Oct-03  &  R3000  &   1200  \\
ASASSN-14ha           &  2014-Oct-09  &  B3000  &   1200  \\
ASASSN-14ha           &  2014-Oct-09  &  R3000  &   1200  \\
ASASSN-14ha           &  2014-Oct-18  &  B3000  &   1200  \\
ASASSN-14ha           &  2014-Oct-18  &  R3000  &   1200  \\
ASASSN-14ha           &  2014-Oct-27  &  B3000  &   1200  \\
ASASSN-14ha           &  2014-Oct-27  &  R3000  &   1200  \\
ASASSN-14hr           &  2014-Oct-03  &  B3000  &   1200  \\
ASASSN-14hr           &  2014-Oct-03  &  R3000  &   1200  \\
ASASSN-14hu           &  2014-Nov-06  &  B3000  &   1200  \\
ASASSN-14hu           &  2014-Nov-06  &  R3000  &   1200  \\
ASASSN-14hu           &  2014-Oct-03  &  B3000  &   1200  \\
ASASSN-14hu           &  2014-Oct-03  &  R3000  &   1200  \\
ASASSN-14hu           &  2014-Oct-09  &  B3000  &   1200  \\
ASASSN-14hu           &  2014-Oct-09  &  R3000  &   1200  \\
ASASSN-14hu           &  2014-Oct-18  &  B3000  &   1200  \\
ASASSN-14hu           &  2014-Oct-18  &  R3000  &   1200  \\
ASASSN-14hu           &  2014-Oct-27  &  B3000  &   1200  \\
ASASSN-14hu           &  2014-Oct-27  &  R3000  &   1200  \\
ASASSN-14ig           &  2014-Oct-03  &  B3000  &   1200  \\
ASASSN-14ig           &  2014-Oct-03  &  R3000  &   1200  \\
ASASSN-14ih           &  2014-Oct-03  &  B3000  &   1200  \\
ASASSN-14ih           &  2014-Oct-03  &  R3000  &   1200  \\
ASASSN-14ii           &  2014-Oct-03  &  B3000  &   1200  \\
ASASSN-14ii           &  2014-Oct-03  &  R3000  &   1200  \\
ASASSN-14il           &  2014-Oct-03  &  B3000  &   1200  \\
ASASSN-14il           &  2014-Oct-03  &  R3000  &   1200  \\
ASASSN-14il           &  2014-Oct-09  &  B3000  &   1200  \\
ASASSN-14il           &  2014-Oct-09  &  R3000  &   1200  \\
ASASSN-14il           &  2014-Oct-18  &  B3000  &   1200  \\
ASASSN-14il           &  2014-Oct-18  &  R3000  &   1200  \\
ASASSN-14il           &  2014-Oct-27  &  B3000  &   1200  \\
ASASSN-14il           &  2014-Oct-27  &  R3000  &   1200  \\
ASASSN-14jc           &  2014-Nov-06  &  B3000  &   1200  \\
ASASSN-14jc           &  2014-Nov-06  &  R3000  &   1200  \\
ASASSN-14jc           &  2014-Oct-27  &  B3000  &   1200  \\
ASASSN-14jc           &  2014-Oct-27  &  R3000  &   1200  \\
ASASSN-14jg           &  2014-Nov-06  &  B3000  &   1200  \\
ASASSN-14jg           &  2014-Nov-06  &  R3000  &   1200  \\
ASASSN-14ko           &  2014-Dec-16  &  B3000  &   1200  \\
ASASSN-14ko           &  2014-Dec-16  &  R7000  &   1200  \\
ASASSN-14ko           &  2015-Feb-15  &  B3000  &   1200  \\
ASASSN-14ko           &  2015-Feb-15  &  R3000  &   1200  \\
ASASSN-14ko           &  2015-Jan-15  &  B3000  &   1200  \\
ASASSN-14ko           &  2015-Jan-15  &  R7000  &   1200  \\
ASASSN-14kp           &  2014-Nov-26  &  B3000  &   1200  \\
ASASSN-14kp           &  2014-Nov-26  &  R3000  &   1200  \\
ASASSN-14kq           &  2014-Nov-26  &  B3000  &   1200  \\
ASASSN-14kq           &  2014-Nov-26  &  R3000  &   1200  \\
ASASSN-14lp           &  2015-Apr-29  &  B3000  &   1200  \\
ASASSN-14lp           &  2015-Apr-29  &  R3000  &   1200  \\
ASASSN-14lp           &  2015-Jul-01  &  B3000  &   1200  \\
ASASSN-14lp           &  2015-Jul-01  &  R3000  &   1200  \\
ASASSN-14lt           &  2014-Dec-16  &  B3000  &   1200  \\
ASASSN-14lt           &  2014-Dec-16  &  R3000  &   1200  \\
ASASSN-14lw           &  2014-Dec-16  &  B3000  &   1200  \\
ASASSN-14lw           &  2014-Dec-16  &  R3000  &   1200  \\
ASASSN-14lw           &  2015-Feb-15  &  B3000  &   1200  \\
ASASSN-14lw           &  2015-Feb-15  &  R3000  &   1200  \\
ASASSN-14lw           &  2015-Jan-06  &  B3000  &   1200  \\
ASASSN-14lw           &  2015-Jan-06  &  R3000  &   1200  \\
ASASSN-14lw           &  2015-Jun-24  &  B3000  &   1200  \\
ASASSN-14lw           &  2015-Jun-24  &  R3000  &   1200  \\
ASASSN-15aj           &  2015-Feb-15  &  B3000  &   1200  \\
ASASSN-15aj           &  2015-Feb-15  &  R3000  &   1200  \\
ASASSN-15aj           &  2015-Feb-24  &  B3000  &   1200  \\
ASASSN-15aj           &  2015-Feb-24  &  R3000  &   1200  \\
ASASSN-15aj           &  2015-Mar-05  &  B3000  &   1200  \\
ASASSN-15aj           &  2015-Mar-05  &  R3000  &   1200  \\
ASASSN-15al           &  2015-Jan-15  &  B3000  &   1200  \\
ASASSN-15al           &  2015-Jan-15  &  R7000  &   1200  \\
ASASSN-15as           &  2015-Jan-16  &  B3000  &   1200  \\
ASASSN-15as           &  2015-Jan-16  &  R7000  &   1200  \\
ASASSN-15az           &  2015-Jan-16  &  B3000  &   1200  \\
ASASSN-15az           &  2015-Jan-16  &  R7000  &   1200  \\
ASASSN-15ba           &  2015-Feb-15  &  B3000  &   1200  \\
ASASSN-15ba           &  2015-Feb-15  &  R3000  &   1200  \\
ASASSN-15ba           &  2015-Feb-24  &  B3000  &   1200  \\
ASASSN-15ba           &  2015-Feb-24  &  R3000  &   1200  \\
ASASSN-15ba           &  2015-Jan-25  &  B3000  &   1200  \\
ASASSN-15ba           &  2015-Jan-25  &  R3000  &   1200  \\
ASASSN-15ba           &  2015-Jan-29  &  B3000  &   1200  \\
ASASSN-15ba           &  2015-Jan-29  &  R3000  &   1200  \\
ASASSN-15ba           &  2015-Jul-08  &  B3000  &   1200  \\
ASASSN-15ba           &  2015-Jul-08  &  R3000  &   1200  \\
ASASSN-15ba           &  2015-Mar-12  &  B3000  &   1200  \\
ASASSN-15ba           &  2015-Mar-12  &  R3000  &   1200  \\
ASASSN-15dz           &  2015-Mar-05  &  B3000  &   1200  \\
ASASSN-15dz           &  2015-Mar-05  &  R3000  &   1200  \\
ASASSN-15eb           &  2015-Mar-05  &  B3000  &   1200  \\
ASASSN-15eb           &  2015-Mar-05  &  R3000  &   1200  \\
ASASSN-15ek           &  2015-Mar-12  &  B3000  &   1200  \\
ASASSN-15ek           &  2015-Mar-12  &  R3000  &   1200  \\
ASASSN-15go           &  2015-Apr-11  &  B3000  &   1200  \\
ASASSN-15go           &  2015-Apr-11  &  R3000  &   1200  \\
ASASSN-15hs           &  2015-Apr-29  &  B3000  &   1200  \\
ASASSN-15hs           &  2015-Apr-29  &  R3000  &   1200  \\
ASASSN-15hx           &  2015-Apr-29  &  B3000  &   1200  \\
ASASSN-15hx           &  2015-Apr-29  &  R3000  &   1200  \\
ASASSN-15hx           &  2015-Aug-17  &  B3000  &    600  \\
ASASSN-15hx           &  2015-Aug-17  &  R3000  &    600  \\
ASASSN-15hx           &  2015-Jul-08  &  B3000  &   1200  \\
ASASSN-15hx           &  2015-Jul-08  &  R3000  &   1200  \\
ASASSN-15hx           &  2015-Jul-31  &  B3000  &   1200  \\
ASASSN-15hx           &  2015-Jul-31  &  R3000  &   1200  \\
ASASSN-15hx           &  2015-Jun-24  &  B3000  &   1200  \\
ASASSN-15hx           &  2015-Jun-24  &  R3000  &   1200  \\
ASASSN-15hy           &  2015-Apr-29  &  B3000  &   1200  \\
ASASSN-15hy           &  2015-Apr-29  &  R3000  &   1200  \\
ASASSN-15hy           &  2015-Aug-17  &  B3000  &   1200  \\
ASASSN-15hy           &  2015-Aug-17  &  R3000  &   1200  \\
ASASSN-15hy           &  2015-Jul-01  &  B3000  &   1200  \\
ASASSN-15hy           &  2015-Jul-01  &  R3000  &   1200  \\
ASASSN-15hy           &  2015-Jul-08  &  B3000  &   1200  \\
ASASSN-15hy           &  2015-Jul-08  &  R3000  &   1200  \\
ASASSN-15hy           &  2015-Jul-31  &  B3000  &   1200  \\
ASASSN-15hy           &  2015-Jul-31  &  R3000  &   1200  \\
ASASSN-15hy           &  2015-Jun-24  &  B3000  &   1200  \\
ASASSN-15hy           &  2015-Jun-24  &  R3000  &   1200  \\
ASASSN-15hy           &  2015-May-03  &  B3000  &    900  \\
ASASSN-15hy           &  2015-May-03  &  R3000  &    900  \\
ASASSN-15hy           &  2015-May-07  &  B3000  &   1200  \\
ASASSN-15hy           &  2015-May-07  &  R3000  &   1200  \\
ASASSN-15hy           &  2015-May-13  &  B3000  &    600  \\
ASASSN-15hy           &  2015-May-13  &  R3000  &    600  \\
ASASSN-15hz           &  2015-Apr-29  &  B3000  &   1200  \\
ASASSN-15hz           &  2015-Apr-29  &  R3000  &   1200  \\
ASASSN-15ic           &  2015-Apr-29  &  B3000  &   1200  \\
ASASSN-15ic           &  2015-Apr-29  &  R3000  &   1200  \\
ASASSN-15lh           &  2015-Jul-01  &  B3000  &   1200  \\
ASASSN-15lh           &  2015-Jul-01  &  R3000  &   1200  \\
ASASSN-15lh           &  2015-Jul-08  &  B3000  &   1200  \\
ASASSN-15lh           &  2015-Jul-08  &  R3000  &   1200  \\
ASASSN-15lh           &  2015-Jul-31  &  B3000  &   1200  \\
ASASSN-15lh           &  2015-Jul-31  &  R3000  &   1200  \\
ASASSN-15lh           &  2015-Jun-24  &  B3000  &   1200  \\
ASASSN-15lh           &  2015-Jun-24  &  R3000  &   1200  \\
ASASSN-15lv           &  2015-Jul-01  &  B3000  &   1200  \\
ASASSN-15lv           &  2015-Jul-01  &  R3000  &   1200  \\
CSS1222               &  2014-Apr-02  &  B3000  &   1200  \\
CSS1222               &  2014-Apr-02  &  R3000  &   1200  \\
Gaia15agm             &  2015-Jul-01  &  B3000  &   1200  \\
Gaia15agm             &  2015-Jul-01  &  R3000  &   1200  \\
LSQ12dlf              &  2012-Aug-11  &  B3000  &   1200  \\
LSQ12dlf              &  2012-Aug-11  &  R3000  &   1200  \\
LSQ12dlf              &  2012-Aug-12  &  B3000  &   1200  \\
LSQ12dlf              &  2012-Aug-12  &  R3000  &   1200  \\
LSQ12dlf              &  2012-Aug-13  &  B3000  &   1200  \\
LSQ12dlf              &  2012-Aug-13  &  R3000  &   1200  \\
LSQ12ege              &  2012-Aug-11  &  B3000  &   1200  \\
LSQ12ege              &  2012-Aug-11  &  R3000  &   1200  \\
LSQ12ege              &  2012-Aug-12  &  B3000  &   1200  \\
LSQ12ege              &  2012-Aug-12  &  R3000  &   1200  \\
LSQ12ege              &  2012-Aug-13  &  B3000  &   1200  \\
LSQ12ege              &  2012-Aug-13  &  R3000  &   1200  \\
LSQ12ehh              &  2012-Aug-11  &  B3000  &   1200  \\
LSQ12ehh              &  2012-Aug-11  &  R3000  &   1200  \\
LSQ12ehh              &  2012-Aug-12  &  B3000  &   1200  \\
LSQ12ehh              &  2012-Aug-12  &  R3000  &   1200  \\
LSQ12ehh              &  2012-Aug-13  &  B3000  &   1200  \\
LSQ12ehh              &  2012-Aug-13  &  R3000  &   1200  \\
LSQ12ers              &  2012-Sep-06  &  B3000  &   1200  \\
LSQ12ers              &  2012-Sep-06  &  R3000  &   1200  \\
LSQ12euu              &  2012-Sep-06  &  B3000  &   1200  \\
LSQ12euu              &  2012-Sep-06  &  R3000  &   1200  \\
LSQ12eve              &  2012-Sep-06  &  B3000  &   1200  \\
LSQ12eve              &  2012-Sep-06  &  R3000  &   1200  \\
LSQ12gdj              &  2012-Nov-19  &  B3000  &   1200  \\
LSQ12gdj              &  2012-Nov-19  &  R3000  &   1200  \\
LSQ12gdj              &  2012-Nov-20  &  B3000  &   1200  \\
LSQ12gdj              &  2012-Nov-20  &  R3000  &   1200  \\
LSQ12gdj              &  2012-Nov-21  &  B3000  &   1200  \\
LSQ12gdj              &  2012-Nov-21  &  R3000  &   1200  \\
LSQ13anm              &  2013-May-26  &  B3000  &   1200  \\
LSQ13anm              &  2013-May-26  &  R3000  &   1200  \\
LSQ13ddu              &  2013-Dec-06  &  B3000  &   1200  \\
LSQ13ddu              &  2013-Dec-06  &  R3000  &   1200  \\
LSQ13ddu              &  2013-Dec-15  &  B3000  &   1200  \\
LSQ13ddu              &  2013-Dec-15  &  R3000  &   1200  \\
LSQ13ddu              &  2013-Dec-19  &  B3000  &   1200  \\
LSQ13ddu              &  2013-Dec-19  &  R3000  &   1200  \\
LSQ13pp               &  2013-Mar-25  &  B3000  &   1200  \\
LSQ13pp               &  2013-Mar-25  &  R3000  &   1200  \\
LSQ14bcj              &  2014-Apr-23  &  B3000  &   1200  \\
LSQ14bcj              &  2014-Apr-23  &  R3000  &   1200  \\
LSQ14bcj              &  2014-Apr-23  &  R7000  &   1200  \\
LSQ15adm              &  2015-Apr-29  &  B3000  &   1200  \\
LSQ15adm              &  2015-Apr-29  &  R3000  &   1200  \\
LSQ15adm              &  2015-Aug-17  &  B3000  &   1200  \\
LSQ15adm              &  2015-Aug-17  &  R3000  &   1200  \\
LSQ15adm              &  2015-Jul-01  &  B3000  &   1200  \\
LSQ15adm              &  2015-Jul-01  &  R3000  &   1200  \\
LSQ15adm              &  2015-Jul-08  &  B3000  &   1200  \\
LSQ15adm              &  2015-Jul-08  &  R3000  &   1200  \\
LSQ15adm              &  2015-Jul-31  &  B3000  &   1200  \\
LSQ15adm              &  2015-Jul-31  &  R3000  &   1200  \\
LSQ15adm              &  2015-Jun-24  &  B3000  &   1060  \\
LSQ15adm              &  2015-Jun-24  &  R3000  &   1060  \\
LSQ15adm              &  2015-May-07  &  B3000  &   1330  \\
LSQ15adm              &  2015-May-07  &  R3000  &   1330  \\
LSQ15adm              &  2015-May-14  &  B3000  &   1800  \\
LSQ15adm              &  2015-May-14  &  R3000  &   1800  \\
LSQ15ey               &  2015-Jan-29  &  B3000  &   1200  \\
LSQ15ey               &  2015-Jan-29  &  R3000  &   1200  \\
MASTERJ1408           &  2014-Apr-23  &  B3000  &   1200  \\
MASTERJ1408           &  2014-Apr-23  &  R7000  &   1200  \\
MASTERJ1353           &  2015-Mar-05  &  B3000  &   1200  \\
MASTERJ1353           &  2015-Mar-05  &  R3000  &   1200  \\
MASTERJ0746           &  2015-Apr-29  &  B3000  &   1200  \\
MASTERJ0746           &  2015-Apr-29  &  R3000  &   1200  \\
OGLE-2013-SN-070      &  2013-Oct-08  &  B3000  &   1200  \\
OGLE-2013-SN-070      &  2013-Oct-08  &  R3000  &   1200  \\
OGLE-2014-SN-019      &  2014-Feb-24  &  B3000  &   1200  \\
OGLE-2014-SN-019      &  2014-Feb-24  &  R3000  &   1200  \\
OGLE-2014-SN-019      &  2014-Mar-14  &  B3000  &   1200  \\
OGLE-2014-SN-019      &  2014-Mar-14  &  R3000  &   1200  \\
OGLE-2014-SN-021      &  2014-Feb-24  &  B3000  &   1200  \\
OGLE-2014-SN-021      &  2014-Feb-24  &  R3000  &   1200  \\
OGLE-2014-SN-021      &  2014-Mar-14  &  B3000  &   1200  \\
OGLE-2014-SN-021      &  2014-Mar-14  &  R3000  &   1200  \\
OGLE-2014-SN-067      &  2014-Aug-29  &  B3000  &   1200  \\
OGLE-2014-SN-067      &  2014-Aug-29  &  R3000  &   1200  \\
PS1-14lz              &  2014-Feb-24  &  B3000  &   1200  \\
PS1-14lz              &  2014-Feb-24  &  R3000  &   1200  \\
PS1-14md              &  2014-Feb-24  &  B3000  &   1200  \\
PS1-14md              &  2014-Feb-24  &  R3000  &   1200  \\
PS1-14ra              &  2014-Mar-14  &  B3000  &   1200  \\
PS1-14ra              &  2014-Mar-14  &  R3000  &   1200  \\
PS1-14vw              &  2014-Apr-02  &  B3000  &   1200  \\
PS1-14vw              &  2014-Apr-02  &  R3000  &   1200  \\
PS1-14vx              &  2014-Apr-02  &  B3000  &   1200  \\
PS1-14vx              &  2014-Apr-02  &  R3000  &   1200  \\
PS1-14wl              &  2014-Apr-02  &  B3000  &   1200  \\
PS1-14wl              &  2014-Apr-02  &  R3000  &   1200  \\
PS15ae                &  2015-Feb-24  &  B3000  &   1200  \\
PS15ae                &  2015-Feb-24  &  R3000  &   1200  \\
PS15ae                &  2015-Mar-12  &  B3000  &   1200  \\
PS15ae                &  2015-Mar-12  &  R3000  &   1200  \\
PS15br                &  2015-Mar-12  &  B3000  &   1200  \\
PS15br                &  2015-Mar-12  &  R3000  &   1200  \\
PSNJ02454138-0812301  &  2014-Oct-27  &  B3000  &   1200  \\
PSNJ02454138-0812301  &  2014-Oct-27  &  R3000  &   1200  \\
PSNJ05031639-0256110  &  2014-Nov-06  &  B3000  &   1200  \\
PSNJ05031639-0256110  &  2014-Nov-06  &  R3000  &   1200  \\
PSNJ09023787+2556042  &  2015-Apr-11  &  B3000  &   1200  \\
PSNJ09023787+2556042  &  2015-Apr-11  &  R3000  &   1200  \\
PSNJ09204691-0803340  &  2014-Dec-16  &  B3000  &   1200  \\
PSNJ09204691-0803340  &  2014-Dec-16  &  R7000  &   1200  \\
PSNJ09204691-0803340  &  2014-Nov-26  &  B3000  &   1200  \\
PSNJ09204691-0803340  &  2014-Nov-26  &  R3000  &   1200  \\
PSNJ09204691-0803340  &  2015-Feb-15  &  B3000  &   1200  \\
PSNJ09204691-0803340  &  2015-Feb-15  &  R3000  &   1200  \\
PSNJ09204691-0803340  &  2015-Jan-15  &  B3000  &   1200  \\
PSNJ09204691-0803340  &  2015-Jan-15  &  R7000  &   1200  \\
PSNJ09204691-0803340  &  2015-Jan-16  &  B3000  &   1200  \\
PSNJ09204691-0803340  &  2015-Jan-16  &  R7000  &   1200  \\
PSNJ10433393-3048206  &  2015-Feb-15  &  B3000  &   1200  \\
PSNJ10433393-3048206  &  2015-Feb-15  &  R3000  &   1200  \\
PSNJ11484578-2817312  &  2013-Dec-06  &  B3000  &   1200  \\
PSNJ11484578-2817312  &  2013-Dec-06  &  R3000  &   1200  \\
PSNJ13471211-2422171  &  2015-Feb-15  &  B3000  &   1200  \\
PSNJ13471211-2422171  &  2015-Feb-15  &  R3000  &   1200  \\
PSNJ17194328-7721305  &  2013-Aug-30  &  B3000  &   1200  \\
PSNJ17194328-7721305  &  2013-Aug-30  &  R3000  &   1200  \\
PSNJ17194328-7721305  &  2013-Aug-30  &  R7000  &   1200  \\
PSNJ17194328-7721305  &  2014-Sep-09  &  B3000  &   1200  \\
PSNJ17194328-7721305  &  2014-Sep-09  &  R3000  &   1200  \\
PSNJ17285509-6609103  &  2013-Aug-30  &  B3000  &   1200  \\
PSNJ17285509-6609103  &  2013-Aug-30  &  R3000  &   1200  \\
PSNJ19251269-5336028  &  2015-Aug-17  &  B3000  &   1200  \\
PSNJ19251269-5336028  &  2015-Aug-17  &  R3000  &   1200  \\
PSNJ20250386-2449133  &  2014-Nov-06  &  B3000  &   1200  \\
PSNJ20250386-2449133  &  2014-Nov-06  &  R3000  &   1200  \\
PSNJ20250386-2449133  &  2014-Nov-14  &  B3000  &   1200  \\
PSNJ20250386-2449133  &  2014-Nov-14  &  R3000  &   1200  \\
PSNJ23320218-4545032  &  2012-Sep-07  &  B3000  &   1200  \\
PSNJ23320218-4545032  &  2012-Sep-07  &  R3000  &   1200  \\
PTF12gzk              &  2012-Aug-10  &  B3000  &   1200  \\
PTF12gzk              &  2012-Aug-10  &  R3000  &   1200  \\
PTF12gzk              &  2012-Aug-11  &  B3000  &   1200  \\
PTF12gzk              &  2012-Aug-11  &  R3000  &   1200  \\
PTF12gzk              &  2012-Aug-12  &  B3000  &   1200  \\
PTF12gzk              &  2012-Aug-12  &  R3000  &   1200  \\
PTF12gzk              &  2012-Aug-13  &  B3000  &   1200  \\
PTF12gzk              &  2012-Aug-13  &  R3000  &   1200  \\
PTF12gzk              &  2012-Sep-06  &  B3000  &   1200  \\
PTF12gzk              &  2012-Sep-06  &  R3000  &   1200  \\
PTF12gzk              &  2012-Sep-07  &  B3000  &   1200  \\
PTF12gzk              &  2012-Sep-07  &  R3000  &   1200  \\
PTF12gzk              &  2012-Sep-23  &  B3000  &   1200  \\
PTF12gzk              &  2012-Sep-23  &  R3000  &   1200  \\
iPTF13bvn             &  2013-Jun-22  &  B3000  &   1200  \\
iPTF13bvn             &  2013-Jun-22  &  R3000  &   1200  \\
iPTF13dge             &  2013-Dec-06  &  B3000  &   1200  \\
iPTF13dge             &  2013-Dec-06  &  R3000  &   1200  \\
iPTF13dge             &  2013-Oct-08  &  B3000  &   1200  \\
iPTF13dge             &  2013-Oct-08  &  R3000  &   1200  \\
iPTF13dge             &  2013-Oct-16  &  B3000  &   1200  \\
iPTF13dge             &  2013-Oct-16  &  R3000  &   1200  \\
iPTF13dge             &  2013-Sep-13  &  B3000  &   1200  \\
iPTF13dge             &  2013-Sep-13  &  R3000  &   1200  \\
iPTF13dge             &  2013-Sep-19  &  B3000  &   1200  \\
iPTF13dge             &  2013-Sep-19  &  R3000  &   1200  \\
iPTF13dge             &  2013-Sep-19  &  R7000  &   1200  \\
SMTJ10310056-3658262  &  2015-Apr-11  &  B3000  &   1200  \\
SMTJ10310056-3658262  &  2015-Apr-11  &  R3000  &   1200  \\
SMTJ03253351-5344190  &  2013-Dec-06  &  B3000  &   1200  \\
SMTJ03253351-5344190  &  2013-Dec-06  &  R3000  &   1200  \\
SMTJ05451320-4735425  &  2014-Jan-13  &  B3000  &    900  \\
SMTJ05451320-4735425  &  2014-Jan-13  &  R3000  &    900  \\
SMTJ13494831-0658174  &  2015-Aug-17  &  B3000  &    900  \\
SMTJ13494831-0658174  &  2015-Aug-17  &  R7000  &    900  \\
SNhunt222             &  2013-Dec-19  &  B3000  &   1200  \\
SNhunt222             &  2013-Dec-19  &  R3000  &   1200  \\
SNhunt239             &  2014-Apr-02  &  B3000  &   1200  \\
SNhunt239             &  2014-Apr-02  &  R3000  &   1200  \\
SNhunt259             &  2014-Oct-18  &  B3000  &   1200  \\
SNhunt259             &  2014-Oct-18  &  R3000  &   1200  \\
SNhunt261             &  2014-Oct-27  &  B3000  &   1200  \\
SNhunt261             &  2014-Oct-27  &  R3000  &   1200  \\
%------------------
\normalsize
\enddata
\end{deluxetable}
%
%
%
% NOT PART OF MAIN SAMPLE
%PSNJ00150879-3912504  &  2014-Oct-07  &  B3000  &   1200  \\
%PSNJ00150879-3912504  &  2014-Oct-07  &  R3000  &   1200  \\
%PSNJ00150879-3912504  &  2014-Oct-09  &  B3000  &   1200  \\
%PSNJ00150879-3912504  &  2014-Oct-09  &  R3000  &   1200  \\
%PSNJ0031              &  2015-Jul-31  &  B3000  &   1200  \\
%PSNJ0031              &  2015-Jul-31  &  R3000  &   1200  \\
%PSNJ1944              &  2014-Mar-04  &  B3000  &   1200  \\
%PSNJ1944              &  2014-Mar-04  &  R3000  &   1200  \\
%PSNJ2316              &  2014-Oct-03  &  B3000  &   1200  \\
%PSNJ2316              &  2014-Oct-03  &  R3000  &   1200  \\


==> table_awsnap_targets.tex <==
\begin{landscape}
\begin{deluxetable}{lllllllllllc}
\tablewidth{0pt}
\tablecaption{All AWSNAP Targets
\label{tab:awsnap_targets}}
\tabletypesize{\small}
\tablehead{
%---------
\colhead{SN} & 
\multicolumn{5}{c}{Discovery} &
\multicolumn{6}{c}{Classification}\\
%---------
\colhead{} & % SN
% Discovery details
\colhead{RA} & 
\colhead{DEC} & 
\colhead{Ref.$^a$} & 
\colhead{Date} & 
\colhead{Group$^b$} & 
% Classification details
\colhead{Ref.} & 
\colhead{Date} & 
\colhead{Group$^c$} & 
\colhead{SN Type} & 
\colhead{Redshift} & 
\colhead{Phase$^d$}
}
\startdata
%#------------------------------------------------------------------------------------------------------------------------------------------------------------------
%# SN                     RA            DEC           DISC-R    DISC-D       DISC-G         CLAS-R     CLAS-D       CLAS-G         TYPE          z            PHASE
%#------------------------------------------------------------------------------------------------------------------------------------------------------------------
SN~2009ip             &  22:23:08.1  &  -28:56:35  &  A4334  &  20120724  &  CRTS        &  A4338   &  20120826  &  Foley            &  SNIIn      &  0.005944  &  (unk)   \\
SN~2012ca             &  18:41:06.5  &  -41:47:38  &  C3101  &  20120426  &  Parker      &  A4076   &  20120429  &  PESSTO           &  SNIIn      &  0.019000  &  (unk)   \\
SN~2012dj             &  23:14:47.2  &  -43:36:22  &  C3167  &  20120702  &  Parker      &  C3167   &  20120706  &  Parrent          &  SNIb/c     &  0.005324  &  +0      \\
SN~2012dn             &  20:23:36.3  &  -28:16:43  &  C3174  &  20120708  &  Parker      &  A4253   &  20120712  &  SNF              &  SNIa       &  0.010187  &  -10     \\
SN~2012dt             &  00:56:38.1  &  -09:53:59  &  C3188  &  20120718  &  Parker      &  A4269   &  20120721  &  PTF              &  SNII       &  0.018900  &  +9      \\
SN~2012dy             &  21:18:49.5  &  -57:38:42  &  C3197  &  20120804  &  Bock        &  C3197   &  20120805  &  Milisavljevic    &  SNII       &  0.010300  &  (young) \\
SN~2012ec             &  02:45:59.9  &  -07:34:15  &  C3201  &  20120811  &  Monard      &  A4306   &  20120812  &  AWSNAP           &  SNII       &  0.004693  &  (young) \\
SN~2012eq             &  01:00:14.5  &  -30:48:26  &  C3223  &  20120827  &  CRTS        &  A4362   &  20120907  &  PESSTO           &  SNIa       &  0.032230  &  +45     \\
SN~2012eu             &  03:13:04.2  &  -08:23:24  &  C3231  &  20120827  &  CRTS        &  C3231   &  20120904  &  Yang             &  SNIa       &  0.030000  &  +30     \\
SN~2012fr             &  03:33:37.1  &  -36:07:28  &  A4523  &  20121027  &  TAROT       &  A4525   &  20121028  &  AWSNAP           &  SNIa       &  0.005400  &  -11     \\
SN~2012hr             &  06:21:37.7  &  -59:42:39  &  C3346  &  20121216  &  Marples     &  A4663   &  20121220  &  Morrell          &  SNIa       &  0.008000  &  -8      \\
SN~2013K              &  17:39:33.1  &  -85:18:18  &  C3391  &  20130120  &  Parker      &  A4754   &  20130121  &  PESSTO           &  SNII       &  0.008000  &  +2      \\
SN~2013aa             &  14:32:33.3  &  -44:13:20  &  C3416  &  20130213  &  Parker      &  A4817   &  20130213  &  LCOGT            &  SNIa       &  0.003999  &  -3      \\
SN~2013ai             &  06:16:18.4  &  -21:22:23  &  C3431  &  20130226  &  Conseil     &  A4851   &  20130302  &  PESSTO           &  SNII       &  0.009000  &  +0      \\
SN~2013aj             &  13:54:00.8  &  -07:55:37  &  C3434  &  20130303  &  Contini     &  A4852   &  20130303  &  PESSTO           &  SNIa       &  0.009000  &  -7      \\
SN~2013am             &  11:18:56.3  &  +13:03:56  &  C3440  &  20130321  &  Sugano      &  A4909   &  20130322  &  ASP              &  SNII       &  0.002692  &  (young) \\
SN~2013ao             &  11:44:44.7  &  -20:31:41  &  C3442  &  20130304  &  CRTS        &  A4863   &  20130305  &  PESSTO           &  SNIa       &  0.030000  &  -7      \\
SN~2013bj             &  14:04:19.9  &  -07:03:02  &  C3482  &  20130404  &  ISSP        &  A4975   &  20130412  &  AWSNAP           &  SNII       &  0.030000  &  +44     \\
SN~2013bk             &  09:40:47.6  &  -05:26:07  &  C3483  &  20130407  &  CRTS        &  A4975   &  20130412  &  AWSNAP           &  SNIc       &  0.020000  &  +3      \\
SN~2013by             &  16:59:01.5  &  -60:11:22  &  C3506  &  20130423  &  Parker      &  C3506   &  20130424  &  Morrell          &  SNII       &  0.003816  &  (young) \\
SN~2013bz             &  13:26:50.7  &  -10:01:39  &  C3507  &  20130421  &  CRTS        &  C3507   &  20130430  &  Chen             &  SNIa-SC    &  0.015000  &  +0      \\
SN~2013cg             &  09:26:57.3  &  -24:47:01  &  C3517  &  20130506  &  CHASE       &  A5057   &  20130508  &  LCOGT            &  SNIa       &  0.007952  &  -7      \\
SN~2013cs             &  13:15:14.2  &  -17:57:56  &  C3533  &  20130512  &  LSQ         &  A5067   &  20130514  &  LSQ              &  SNIa       &  0.009240  &  -7      \\
SN~2013cy             &  22:10:33.5  &  -22:39:48  &  C3546  &  20130531  &  Monard/LSQ  &  A5100   &  20130603  &  AWSNAP           &  SNIa       &  0.034000  &  +0      \\
SN~2013cz             &  19:49:32.5  &  -70:12:59  &  C3547  &  20130507  &  Parker      &  A5101   &  20130603  &  AWSNAP           &  SNII       &  0.015000  &  +21     \\
SN~2013df             &  12:26:28.1  &  +31:13:50  &  C3557  &  20130607  &  ISSP        &  C3557   &  20130610  &  Cenko            &  SNIIb      &  0.002388  &  (young) \\
SN~2013dh             &  15:30:00.3  &  +12:59:27  &  C3561  &  20130612  &  LOSS        &  C3561   &  20130614  &  Cenko            &  SNIa-91T   &  0.013356  &  -5      \\
SN~2013du             &  01:24:13.6  &  -34:43:27  &  C3579  &  20130623  &  Parker      &  A5194   &  20130704  &  AWSNAP           &  SNII       &  0.019000  &  +30     \\
SN~2013ef             &  01:55:20.2  &  +06:36:35  &  A5193  &  20130704  &  ASAS-SN     &  A5194   &  20130704  &  AWSNAP           &  SNIa       &  0.015000  &  +0      \\
SN~2013ej             &  01:36:48.2  &  +15:45:35  &  C3606  &  20130725  &  LOSS        &  A5228   &  20130727  &  LCOGT            &  SNII       &  0.002192  &  (young) \\
SN~2013ek             &  20:57:54.2  &  -51:52:10  &  C3607  &  20130724  &  Parker      &  A5227   &  20130725  &  LCOGT            &  SNIb       &  0.016000  &  +5      \\
SN~2013er             &  13:07:51.2  &  -00:51:54  &  C3619  &  20130729  &  Parker      &  A5238   &  20130731  &  AWSNAP           &  SNIa       &  0.018052  &  -4      \\
SN~2013fd             &  01:33:59.6  &  -34:23:38  &  C3645  &  20130827  &  Parker      &  A5345   &  20130829  &  PESSTO           &  SNII       &  0.013000  &  (young) \\
SN~2013fj             &  22:15:28.3  &  +15:34:06  &  C3654  &  20130907  &  ISSP        &  C3654   &  20130913  &  ASP              &  SNIa       &  0.033570  &  +4      \\
SN~2013fq             &  19:59:06.7  &  -55:55:36  &  C3665  &  20130915  &  Parker      &  A5400   &  20130918  &  Hsiao            &  SNIIb      &  0.011300  &  +0      \\
SN~2013fs             &  23:19:44.5  &  +10:10:38  &  C3671  &  20131006  &  Itagaki     &  A5527   &  20131008  &  AWSNAP           &  SNII       &  0.012000  &  (young) \\
SN~2013ft             &  23:41:36.9  &  +03:43:16  &  C3672  &  20130913  &  LOSS        &  A5455   &  20131008  &  AWSNAP           &  SNII       &  0.009600  &  +13     \\
SN~2013fw             &  21:13:44.1  &  +13:34:50  &  C3681  &  20131022  &  Jin,Gao     &  A5507   &  20131024  &  LCOGT            &  SNIa       &  0.016952  &  -14     \\
SN~2013gh             &  22:02:21.8  &  -18:55:00  &  C3706  &  20130808  &  LOSS        &  A5262   &  20130811  &  LCOGT            &  SNIa       &  0.008800  &  -7      \\
SN~2013gi             &  06:23:48.2  &  -65:19:43  &  C3714  &  20131113  &  Parker      &  A5582   &  20131114  &  AWSNAP           &  SNIa       &  0.030100  &  +10     \\
SN~2013gq             &  19:59:07.8  &  -55:55:03  &  C3730  &  20130325  &  LOSS        &  A4940   &  20130402  &  PESSTO           &  SNIa       &  0.014000  &  +0      \\
SN~2013gr             &  01:46:28.5  &  -58:40:25  &  C3733  &  20131128  &  Marples     &  A5612   &  20131130  &  Hsiao            &  SNIax      &  0.007000  &  +0      \\
SN~2013hh             &  11:29:04.8  &  +17:14:08  &  C3754  &  20131111  &  TAROT       &  A5656   &  20131212  &  AWSNAP           &  SNIa-91T   &  0.012000  &  -2      \\
SN~2013hj             &  09:12:05.7  &  -15:25:39  &  C3757  &  20131212  &  CHASE       &  C3757   &  20131213  &  ASP              &  SNII       &  0.006900  &  (young) \\
SN~2013hn             &  13:50:52.3  &  -30:16:54  &  C3762  &  20131213  &  Kot+        &  C3762   &  20131217  &  LCOGT            &  SNIa       &  0.015140  &  -5      \\
SN~2013hu             &  11:28:07.2  &  -13:11:24  &  C3776  &  20131228  &  Itagaki     &  A5716   &  20140101  &  PESSTO           &  SNII       &  0.015000  &  +25     \\
SN~2013hx             &  01:35:33.4  &  -57:57:55  &  C3836  &  20131227  &  SkyMapper   &  A5912   &  20140220  &  PESSTO           &  SLSN       &  0.135000  &  +0      \\
SN~2014D              &  12:10:37.1  &  +18:49:50  &  C3778  &  20140101  &  CRTS        &  A5742   &  20140109  &  ASP              &  SNIa       &  0.008179  &  -2      \\
SN~2014E              &  12:03:31.9  &  +02:02:46  &  C3784  &  20140105  &  PTF         &  A5741   &  20140106  &  PTF              &  SNIa       &  0.018906  &  -3      \\
SN~2014I              &  05:42:20.1  &  -25:32:34  &  C3791  &  20140117  &  Parker      &  A5777   &  20140118  &  AWSNAP           &  SNIa       &  0.030014  &  -1      \\
SN~2014L              &  12:18:48.3  &  +14:24:55  &  C3795  &  20140126  &  TNTS        &  C3795   &  20140127  &  TNTS             &  SNIc       &  0.008029  &  +0      \\
SN~2014N              &  02:30:59.0  &  -44:25:26  &  C3798  &  20140127  &  Parker      &  C3798   &  20140202  &  Drout            &  SNII       &  0.017000  &  +35     \\
SN~2014X              &  12:10:41.3  &  -34:03:28  &  C3820  &  20140301  &  Parker      &  A5948   &  20140304  &  AWSNAP           &  SNIa       &  0.021000  &  +21     \\
SN~2014aa             &  11:45:03.3  &  +19:58:38  &  C3823  &  20140307  &  Arbor       &  A5958   &  20140309  &  ASP              &  SNIa       &  0.016982  &  -7      \\
SN~2014ac             &  15:04:39.7  &  +12:38:02  &  C3830  &  20140310  &  ISSP        &  A5970   &  20140310  &  PESSTO           &  SNIa       &  0.030000  &  +0      \\
SN~2014ad             &  11:57:44.0  &  -10:10:03  &  C3831  &  20140312  &  CRTS        &  C3831   &  20140315  &  Jha              &  SNIc-BL    &  0.005700  &  (young) \\
SN~2014ah             &  11:55:30.4  &  +11:55:28  &  C3835  &  20140312  &  ISSP        &  C3835   &  20140311  &  ASP              &  SNIa       &  0.021026  &  -7      \\
SN~2014ao             &  08:34:33.2  &  -02:32:33  &  C3855  &  20140417  &  LOSS        &  A6077   &  20140417  &  ASP              &  SNIa       &  0.014000  &  -10     \\
SN~2014ap             &  11:30:13.3  &  +24:10:17  &  C3856  &  20140320  &  ISSP        &  A6001   &  20140322  &  AWSNAP           &  SNIa       &  0.023516  &  -1      \\
SN~2014at             &  21:46:13.9  &  -46:31:21  &  C3862  &  20140420  &  Parker      &  A6087   &  20140420  &  PESSTO           &  SNIa       &  0.030000  &  -7      \\
SN~2014au             &  14:19:29.6  &  -05:37:29  &  C3864  &  20140420  &  CRTS        &  A6091   &  20140422  &  PESSTO           &  SNII       &  0.034920  &  +16     \\
SN~2014bx             &  19:43:52.4  &  -70:37:52  &  C3926  &  20140720  &  Parker      &  A6335   &  20140722  &  AWSNAP           &  SNIa       &  0.011570  &  -1      \\
SN~2014bz             &  13:56:04.2  &  -43:35:10  &  C3932  &  20140506  &  Conseil     &  A6230   &  20140611  &  AWSNAP           &  SNIa       &  0.022516  &  +30     \\
SN~2014ca             &  16:53:20.9  &  -72:30:52  &  C3935  &  20140510  &  Parker      &  A6230   &  20140611  &  AWSNAP           &  SNII       &  0.019487  &  +65     \\
SN~2014cm             &  18:08:30.6  &  -52:04:11  &  C3951  &  20140530  &  Parker      &  A6230   &  20140611  &  AWSNAP           &  SNII       &  0.018219  &  +71     \\
SN~2014co             &  01:10:35.5  &  -30:13:33  &  C3953  &  20140621  &  Monard      &  A6302   &  20140708  &  AWSNAP           &  SNII       &  0.019036  &  +10     \\
SN~2014cp             &  02:25:29.7  &  -25:37:36  &  C3954  &  20140623  &  Parker      &  A6302   &  20140708  &  AWSNAP           &  SNIc-BL    &  0.016164  &  +1      \\
SN~2014cq             &  09:23:29.6  &  -63:40:28  &  C3955  &  20140620  &  Parker      &  A6302   &  20140708  &  AWSNAP           &  SNIIb      &  0.010673  &  +20     \\
SN~2014cr             &  19:37:05.5  &  -42:17:44  &  C3956  &  20140627  &  Monard      &  A6302   &  20140708  &  AWSNAP           &  SNIax      &  0.019123  &  +23     \\
SN~2014cs             &  21:35:51.9  &  -62:05:33  &  C3957  &  20140622  &  Parker      &  A6302   &  20140708  &  AWSNAP           &  SNIa       &  0.053664  &  +23     \\
SN~2014ct             &  09:59:25.2  &  -00:15:19  &  C3958  &  20140601  &  Parker      &  A6230   &  20140611  &  AWSNAP           &  SNIa       &  0.047987  &  +24     \\
SN~2014cu             &  21:50:47.1  &  -73:55:27  &  C3959  &  20140622  &  Parker      &  A6302   &  20140708  &  AWSNAP           &  SNII       &  0.028326  &  +20     \\
SN~2014cw             &  22:15:26.7  &  -10:28:40  &  C3962  &  20140829  &  MASTER      &  A6440   &  20140902  &  PESSTO           &  SNII       &  0.006000  &  +0      \\
SN~2014cx             &  00:59:47.9  &  -07:34:26  &  C3963  &  20140902  &  Itagaki     &  A6440   &  20140902  &  PESSTO           &  SNII       &  0.005490  &  (young) \\
SN~2014cy             &  23:44:16.1  &  +10:46:05  &  C3964  &  20140831  &  Nishimura   &  A6437   &  20140902  &  LCOGT            &  SNII       &  0.005547  &  (young) \\
SN~2014dc             &  03:30:54.6  &  -47:58:49  &  C3970  &  20140904  &  Maza        &  C3970   &  20140910  &  Beletsky/AWSNAP  &  SNII       &  0.022436  &  -2      \\
SN~2014df             &  03:44:24.5  &  -44:40:04  &  C3977  &  20140603  &  Monard      &  A6201   &  20140603  &  AWSNAP           &  SNIb       &  0.003896  &  +6      \\
SN~2014dl             &  16:29:46.1  &  +08:38:31  &  C3995  &  20140925  &  CRTS        &  A6507   &  20140926  &  ASP              &  SNIa-91T   &  0.032966  &  -6      \\
SN~2014dn             &  04:17:54.8  &  -56:36:48  &  C3997  &  20140924  &  Parker      &  A6510   &  20140928  &  Morrell          &  SNIa-pec   &  0.022189  &  +3      \\
SN~2014do             &  08:17:47.8  &  -30:07:25  &  C4000  &  20140928  &  Parker      &  A6536   &  20141003  &  AWSNAP           &  SNII       &  0.005520  &  +13     \\
SN~2014dp             &  08:19:38.2  &  -22:34:17  &  C4002  &  20140928  &  Parker      &  A6562   &  20141009  &  AWSNAP           &  SNIb       &  0.018951  &  +11     \\
SN~2014dq             &  22:23:16.4  &  -28:58:34  &  A6592  &  20141019  &  ASAS-SN     &  A6600   &  20141020  &  Challis          &  SNII       &  0.006000  &  (young) \\
SN~2014dr             &  03:22:46.6  &  +00:09:28  &  C4009  &  20141014  &  CRTS        &  A6610   &  20141023  &  ASP              &  SNII       &  0.023000  &  +45     \\
SN~2014eg             &  02:45:09.0  &  -55:44:27  &  A6711  &  20141116  &  PESSTO      &  A6739   &  20141122  &  PESSTO           &  SNIa-91T   &  0.018000  &  -7      \\
SN~2015F              &  07:36:16.3  &  -69:30:17  &  C4081  &  20150309  &  Monard      &  A7209   &  20150310  &  PESSTO           &  SNIa       &  0.004000  &  -11     \\
SN~2015J              &  07:35:07.0  &  -69:08:01  &  C4115  &  20150427  &  SkyMapper   &  A7711   &  20150624  &  AWSNAP           &  SNIIn      &  0.005400  &  (unk)   \\
SN~2015L              &  22:02:14.3  &  -61:39:32  &  A7642  &  20150614  &  ASAS-SN     &  A7774   &  20150621  &  Dong             &  SLSN       &  0.232600  &  (unk)   \\
SN~2015S              &  00:31:26.7  &  -49:35:35  &  C4130  &  20150722  &  Marples     &  A7866   &  20150731  &  AWSNAP           &  SNII       &  0.021912  &  +2      \\
ASASSN-13co           &  21:40:38.5  &  +06:30:40  &  A5346  &  20130829  &  ASAS-SN     &  A5353   &  20130901  &  Morrell          &  SNII       &  0.022600  &  +0      \\
ASASSN-14dp           &  11:21:58.4  &  -37:54:25  &  A6297  &  20140707  &  ASAS-SN     &  A6302   &  20140708  &  AWSNAP           &  SNII       &  0.009159  &  -1      \\
ASASSN-14eu           &  15:00:36.9  &  -03:50:52  &  A6360  &  20140801  &  ASAS-SN     &  A6363   &  20140802  &  Milisavljevic    &  SNIa       &  0.022722  &  +0      \\
ASASSN-14ew           &  20:22:00.7  &  -51:47:48  &  A6367  &  20140804  &  ASAS-SN     &  A6384   &  20140811  &  Takats           &  SNIa       &  0.019597  &  +0      \\
ASASSN-14fo           &  20:34:06.5  &  -01:58:13  &  A6397  &  20140815  &  ASAS-SN     &  A6399   &  20140816  &  PESSTO           &  SNIa       &  0.020000  &  +2      \\
ASASSN-14fw           &  23:49:06.7  &  -07:03:05  &  A6404  &  20140818  &  ASAS-SN     &  A6417   &  20140824  &  PESSTO           &  SNIa       &  0.019000  &  +10     \\
ASASSN-14ha           &  04:20:02.0  &  -54:56:19  &  A6460  &  20140910  &  ASAS-SN     &  A6466   &  20140913  &  LCOGT            &  SNII       &  0.005017  &  (young) \\
ASASSN-14hr           &  01:50:41.6  &  -14:31:08  &  A6500  &  20140925  &  ASAS-SN     &  A6508   &  20140927  &  CSP              &  SNIa       &  0.033620  &  -5      \\
ASASSN-14hu           &  06:43:27.5  &  -69:38:17  &  A6505  &  20140927  &  ASAS-SN     &  A6510   &  20140928  &  CSP              &  SNIa       &  0.015000  &  -5      \\
ASASSN-14ig           &  01:16:05.3  &  -61:37:21  &  A6517  &  20140921  &  ASAS-SN     &  A6536   &  20141003  &  AWSNAP           &  SNIa       &  0.030000  &  +15     \\
ASASSN-14ih           &  22:34:30.4  &  -24:39:54  &  A6521  &  20140919  &  ASAS-SN     &  A6536   &  20141003  &  AWSNAP           &  SNIa       &  0.032000  &  +20     \\
ASASSN-14ii           &  22:16:41.5  &  -36:09:42  &  A6521  &  20140922  &  ASAS-SN     &  A6536   &  20141003  &  AWSNAP           &  SNIa       &  0.030000  &  +9      \\
ASASSN-14il           &  00:45:33.0  &  -14:15:34  &  A6525  &  20141001  &  ASAS-SN     &  A6536   &  20141003  &  AWSNAP           &  SNIIn      &  0.022000  &  (young) \\
ASASSN-14jc           &  07:35:34.7  &  -62:46:10  &  A6594  &  20141019  &  ASAS-SN     &  A6618   &  20141023  &  PESSTO           &  SNIa       &  0.011320  &  +0      \\
ASASSN-14jg           &  23:33:14.5  &  -60:34:13  &  A6637  &  20141021  &  ASAS-SN     &  A6661   &  20141102  &  LCOGT            &  SNIa       &  0.014800  &  +0      \\
ASASSN-14ko           &  05:25:16.5  &  -45:59:24  &  A6732  &  20141114  &  ASAS-SN     &  A6749   &  20141124  &  PESSTO           &  SNIIn      &  0.042000  &  (unk)   \\
ASASSN-14kp           &  00:39:38.6  &  -38:04:38  &  A6736  &  20141122  &  ASAS-SN     &  A6765   &  20141127  &  CSP              &  SNII       &  0.023000  &  +0      \\
ASASSN-14kq           &  23:45:15.5  &  -29:47:01  &  A6737  &  20141123  &  ASAS-SN     &  A6765   &  20141127  &  CSP              &  SNIa       &  0.034000  &  -2      \\
ASASSN-14lp           &  12:45:08.6  &  -00:27:29  &  A6795  &  20141210  &  ASAS-SN     &  A6801   &  20141211  &  Thorstensen      &  SNIa       &  0.005101  &  -3      \\
ASASSN-14lt           &  03:11:07.4  &  -13:06:30  &  A6802  &  20141210  &  ASAS-SN     &  A6804   &  20141212  &  ASP              &  SNIa       &  0.032000  &  -7      \\
ASASSN-14lw           &  01:06:47.6  &  -46:58:55  &  A6809  &  20141212  &  ASAS-SN     &  A6832   &  20141216  &  AWSNAP           &  SNIa-91T   &  0.016000  &  -4      \\
ASASSN-15aj           &  10:52:54.2  &  -32:55:26  &  A6886  &  20150108  &  ASAS-SN     &  A6905   &  20150112  &  Simon            &  SNIa       &  0.010921  &  +1      \\
ASASSN-15al           &  04:57:49.6  &  -21:35:35  &  A6894  &  20150104  &  ASAS-SN     &  A6909   &  20150112  &  PESSTO           &  SNIa       &  0.030000  &  +0      \\
ASASSN-15as           &  09:39:16.8  &  +06:25:56  &  A6919  &  20150113  &  ASAS-SN     &  A6920   &  20150114  &  Morrell          &  SNIa       &  0.030000  &  +0      \\
ASASSN-15az           &  11:08:38.0  &  -10:14:48  &  A6921  &  20150114  &  ASAS-SN     &  A6925   &  20150115  &  ASP              &  SNIa       &  0.028000  &  +0      \\
ASASSN-15ba           &  14:04:55.1  &  +08:55:15  &  A6934  &  20150115  &  ASAS-SN     &  A6947   &  20150115  &  Challis          &  SNIa       &  0.023100  &  -5      \\
ASASSN-15dz           &  16:41:20.9  &  +08:54:32  &  A7145  &  20150221  &  ASAS-SN     &  A7180   &  20150306  &  AWSNAP           &  SNIa       &  0.032216  &  +9      \\
ASASSN-15eb           &  08:06:07.8  &  -22:33:51  &  A7157  &  20150226  &  ASAS-SN     &  A7180   &  20150306  &  AWSNAP           &  SNIa       &  0.016481  &  +8      \\
ASASSN-15go           &  06:11:22.5  &  -16:25:21  &  A7349  &  20150406  &  ASAS-SN     &  A7368   &  20150411  &  AWSNAP           &  SNIa       &  0.018923  &  -4      \\
ASASSN-15hs           &  15:33:34.7  &  -78:07:12  &  A7444  &  20150424  &  ASAS-SN     &  A7458   &  20150429  &  AWSNAP           &  SNIIn      &  0.008900  &  (unk)   \\
ASASSN-15hx           &  13:43:16.7  &  -31:33:21  &  A7447  &  20150426  &  ASAS-SN     &  A7452   &  20150426  &  PESSTO           &  SNIa       &  0.010000  &  -11     \\
ASASSN-15hy           &  20:10:01.6  &  -00:44:16  &  A7450  &  20150425  &  ASAS-SN     &  A7452   &  20150426  &  PESSTO           &  SNIa-pec   &  0.025000  &  -13     \\
ASASSN-15hz           &  22:29:37.8  &  -65:27:44  &  A7450  &  20150426  &  ASAS-SN     &  A7458   &  20150429  &  AWSNAP           &  SNIa       &  0.033000  &  -3      \\
ASASSN-15ic           &  06:14:52.0  &  -42:48:00  &  A7455  &  20150427  &  ASAS-SN     &  A7458   &  20150429  &  AWSNAP           &  SNIa       &  0.025000  &  -1      \\
ASASSN-15lv           &  01:59:01.0  &  -32:22:28  &  A7700  &  20150705  &  ASAS-SN     &  A7746   &  20150701  &  AWSNAP           &  SNIIb      &  0.011000  &  -2      \\
SNhunt222             &  10:00:26.2  &  +03:22:50  &  CTOCP  &  20131214  &  CRTS/LSQ    &  A5860   &  20140207  &  PESSTO           &  SNII       &  0.006860  &  +60     \\
SNhunt239             &  12:09:09.7  &  +31:34:28  &  CTOCP  &  20140325  &  CRTS        &  A6040   &  20140402  &  AWSNAP           &  SNIa-91bg  &  0.022666  &  +10     \\
SNhunt259             &  00:00:21.6  &  -02:36:23  &  CTOCP  &  20141015  &  CRTS        &  (NEW)   &  20141018  &  AWSNAP           &  SNIa       &  0.037909  &  +100    \\
SNhunt261             &  02:45:29.8  &  -17:31:41  &  CTOCP  &  20141017  &  CRTS        &  A6629   &  20141027  &  AWSNAP           &  SNIa-91bg  &  0.029070  &  +2      \\
CSS1222               &  12:22:57.0  &  +28:29:57  &  CRTS   &  20140326  &  CRTS        &  A6040   &  20140402  &  AWSNAP           &  SNII       &  0.024000  &  +2      \\
Gaia15agm             &  23:55:57.6  &  -43:43:40  &  Gaia   &  20150601  &  Gaia        &  A7746   &  20150701  &  AWSNAP           &  SNIa       &  0.029000  &  +31     \\
LSQ12dlf              &  01:50:29.8  &  -21:48:45  &  LSQ    &  20120710  &  LSQ         &  A4329   &  20120818  &  PESSTO           &  SLSN-Ic    &  0.250000  &  +21     \\
LSQ12ege              &  16:50:51.7  &  +02:52:40  &  LSQ    &  20120715  &  LSQ         &  A4303   &  20120809  &  PESSTO           &  SNIa       &  0.080000  &  -5      \\
LSQ12ehh              &  16:27:12.4  &  +02:05:12  &  LSQ    &  20120727  &  LSQ         &  A4303   &  20120809  &  PESSTO           &  SNIa       &  0.100000  &  -6      \\
LSQ12ers              &  23:02:03.3  &  -22:52:17  &  LSQ    &  20120829  &  LSQ         &  A4357   &  20120906  &  AWSNAP           &  SNIa       &  0.099000  &  +1      \\
LSQ12euu              &  21:31:07.5  &  -06:41:49  &  LSQ    &  20120902  &  LSQ         &  A4357   &  20120906  &  AWSNAP           &  SNIa       &  0.116000  &  -1      \\
LSQ12eve              &  21:53:16.7  &  -21:42:45  &  LSQ    &  20120903  &  LSQ         &  A4357   &  20120906  &  AWSNAP           &  SNIa       &  0.098000  &  -7      \\
LSQ12gdj              &  23:54:45.3  &  -25:40:36  &  LSQ    &  20121107  &  LSQ         &  A4566   &  20121110  &  SNF              &  SNIa-91T   &  0.030324  &  -5      \\
LSQ13ddu              &  03:58:48.4  &  -29:24:54  &  LSQ    &  20131122  &  LSQ         &  --      &  20131130  &  PESSTO           &  SLSN       &  0.058000  &  (unk)   \\
LSQ13pp               &  12:42:02.9  &  -22:05:07  &  LSQ    &  20130318  &  LSQ         &  (NEW)   &  20130325  &  AWSNAP           &  SNII       &  0.045700  &  +7      \\
LSQ14bcj              &  14:05:58.2  &  -12:04:12  &  LSQ    &  20140403  &  LSQ         &  A6087   &  20140420  &  PESSTO           &  SNIa       &  0.020000  &  -7      \\
LSQ15adm              &  20:14:20.9  &  -58:08:01  &  LSQ    &  20150405  &  LSQ         &  A7363   &  20150409  &  PESSTO           &  SNIa-csm   &  0.073000  &  +10     \\
LSQ15ey               &  14:12:05.1  &  -07:23:37  &  LSQ    &  20150120  &  LSQ         &  A6994   &  20150125  &  PESSTO           &  SNII       &  0.036000  &  (young) \\
MASTERJ1408           &  14:08:04.9  &  -11:59:46  &  A6084  &  20140330  &  MASTER      &  A6092   &  20140423  &  AWSNAP           &  SNIa       &  0.035308  &  +25     \\
MASTERJ1353           &  13:53:30.3  &  -42:16:19  &  A7151  &  20150227  &  MASTER      &  A7209   &  20150310  &  PESSTO           &  SNIIn      &  0.052000  &  +10     \\
MASTERJ0746           &  07:46:10.7  &  -71:22:20  &  A7451  &  20150426  &  MASTER      &  A7458   &  20150429  &  AWSNAP           &  SNIa       &  0.017400  &  -7      \\
OGLE-2013-SN-070      &  00:45:15.0  &  -66:19:06  &  A5397  &  20130910  &  OGLE        &  A5455   &  20131008  &  AWSNAP           &  SNIa       &  0.043000  &  +33     \\
OGLE-2014-SN-019      &  06:13:50.4  &  -67:55:13  &  A5916  &  20140222  &  OGLE        &  A5915   &  20140222  &  PESSTO           &  SNIa       &  0.040000  &  -3      \\
OGLE-2014-SN-021      &  05:48:25.3  &  -66:47:31  &  A5916  &  20140224  &  OGLE        &  A5919   &  20140224  &  AWSNAP           &  SNIa       &  0.039000  &  +0      \\
OGLE-2014-SN-067      &  04:57:50.4  &  -74:00:40  &  A6423  &  20140815  &  OGLE        &  A6430   &  20140829  &  AWSNAP           &  SNIc       &  0.018700  &  +0      \\
PS1-14lz              &  04:50:48.8  &  -14:25:23  &  PS1    &  20140213  &  PanSTARRS   &  A5908   &  20140219  &  PESSTO           &  SNIa       &  0.070000  &  +1      \\
PS1-14md              &  11:17:42.3  &  -21:14:35  &  PS1    &  20140213  &  PanSTARRS   &  A5919   &  20140224  &  AWSNAP           &  SNIa       &  0.071000  &  +3      \\
PS1-14ra              &  14:41:28.3  &  +09:26:12  &  PS1    &  20140305  &  PanSTARRS   &  A5957   &  20140307  &  PESSTO           &  SNIa       &  0.030000  &  +0      \\
PS1-14vw              &  09:58:07.5  &  +07:57:57  &  PS1    &  20140325  &  PanSTARRS   &  A6040   &  20140402  &  AWSNAP           &  SNIa       &  0.091000  &  +14     \\
PS1-14vx              &  10:41:50.9  &  +16:49:06  &  PS1    &  20140325  &  PanSTARRS   &  A6040   &  20140402  &  AWSNAP           &  SNIa       &  0.057000  &  +23     \\
PS1-14wl              &  13:32:42.0  &  -20:36:24  &  PS1    &  20140325  &  PanSTARRS   &  A6040   &  20140402  &  AWSNAP           &  SNIa       &  0.034000  &  +0      \\
PS15ae                &  11:33:41.7  &  +00:43:40  &  PS1    &  20141223  &  CRTS/PS1    &  A7102   &  20150217  &  PESSTO           &  SLSN-Ic    &  0.110000  &  +0      \\
PS15br                &  11:25:19.2  &  +08:14:18  &  PS1    &  20150215  &  PanSTARRS   &  A7209   &  20150310  &  PESSTO           &  SLSN       &  0.101000  &  (unk)   \\
PSNJ02454138-0812301  &  02:45:41.4  &  -08:12:30  &  CTOCP  &  20141024  &  ISSP        &  A6628   &  20141027  &  ASP              &  SNIa       &  0.029613  &  +3      \\
PSNJ05031639-0256110  &  05:03:16.4  &  -02:56:11  &  CTOCP  &  20141105  &  LOSS        &  A6682   &  20141110  &  Kangas           &  SNIb       &  0.014440  &  +0      \\
PSNJ09023787+2556042  &  09:02:37.9  &  +25:56:04  &  A7366  &  20150411  &  LOSS        &  A7368   &  20150411  &  AWSNAP           &  SNIIb      &  0.008172  &  -3      \\
PSNJ09204691-0803340  &  09:20:46.9  &  -08:03:34  &  CTOCP  &  20141120  &  Gagliano    &  A6734   &  20141121  &  NAOC             &  SNIIn      &  0.019644  &  -10     \\
PSNJ10433393-3048206  &  10:43:33.9  &  -30:48:21  &  CTOCP  &  20150211  &  Parker      &  A7073   &  20150212  &  Morrell          &  SNIIn      &  0.013000  &  +117    \\
PSNJ11484578-2817312  &  11:48:45.8  &  -28:17:31  &  CTOCP  &  20131127  &  CHASE       &  A5615   &  20131129  &  PESSTO           &  SNIc-BL    &  0.010000  &  +20     \\
PSNJ13471211-2422171  &  13:47:12.1  &  -24:22:17  &  CTOCP  &  20150212  &  Parker      &  A7075   &  20150215  &  Stritzinger      &  SNIa       &  0.019910  &  +0      \\
PSNJ17194328-7721305  &  17:19:43.3  &  -77:21:31  &  CTOCP  &  20130825  &  Aldous      &  A5331   &  20130826  &  PESSTO           &  SNIa       &  0.009000  &  -4      \\
PSNJ17285509-6609103  &  17:28:55.1  &  -66:09:10  &  CTOCP  &  20130827  &  Marples     &  A5338   &  20130828  &  PESSTO           &  SNII       &  0.021908  &  +7      \\
PSNJ19251269-5336028  &  19:25:12.7  &  -53:36:03  &  CTOCP  &  20150810  &  Parker      &  A7925   &  20150817  &  AWSNAP           &  SNIa       &  0.054000  &  +48     \\
PSNJ20250386-2449133  &  20:25:04.1  &  -24:49:20  &  A6659  &  20141028  &  LOSS        &  A6667   &  20141104  &  LCOGT            &  SNIc       &  0.010614  &  -3      \\
PSNJ23320218-4545032  &  23:32:02.2  &  -45:45:03  &  CTOCP  &  20120828  &  CRTS        &  (NEW)   &  20120907  &  AWSNAP           &  SNIc       &  0.005000  &  +60     \\
PTF12gzk              &  22:12:41.5  &  +00:30:53  &  A4298  &  20120724  &  PTF         &  A4298   &  20120727  &  PTF              &  SNIc-BL    &  0.013700  &  (young) \\
iPTF13bvn             &  14:59:59.4  &  +01:52:59  &  A5147  &  20130616  &  iPTF        &  A5142   &  20140617  &  Milisavljevic    &  SNIb       &  0.004490  &  -32     \\
iPTF13dge             &  05:03:35.3  &  +01:34:15  &  A5366  &  20130904  &  iPTF        &  A5366   &  20130904  &  PTF              &  SNIa       &  0.015854  &  -15     \\
SMTJ10310056-3658262  &  10:30:40.0  &  -36:57:51  &  A7261  &  20150313  &  SkyMapper   &  A7261   &  20150319  &  PESSTO           &  SNIa       &  0.035000  &  +0      \\
SMTJ03253351-5344190  &  03:25:33.8  &  -53:44:22  &  A5641  &  20131201  &  SkyMapper   &  A5641   &  20131206  &  AWSNAP           &  SNIa       &  0.055000  &  -6      \\
SMTJ05451320-4735425  &  05:45:13.7  &  -47:35:37  &  --     &  20150315  &  SkyMapper   &  --      &  --        &  LCOGT            &  SNIa       &  0.050000  &  +0      \\
SMTJ13494831-0658174  &  13:49:48.0  &  -06:58:17  &  A7925  &  20150728  &  SkyMapper   &  A7925   &  20150817  &  AWSNAP           &  SNIa       &  0.076933  &  +12     \\
%------------------
\enddata
\tablecomments{
$^a$ Notation: A1234 $\equiv$ ATel \# 1234; C1234 $\equiv$ CBET \# 1234; CTOCP $\equiv$ CBET Transient Object Confirmation Page; objects newly classified here denoted as (NEW); all others refer to transient announcement webpages for stated discovery group(s).\\
$^b$ Discovery group acronyms (where appropriate -- see text for details) or lead author of the discovery alert.\\
$^c$ Classifcation group acronyms (where appropriate -- see text for details) or lead author of the classification alert.\\
$^d$ Phase with respect to maximum light (where appropriate) for the best {\em spectroscopic match}, as reported by the classifying group.  SNe IIn do not typically have a clearly identifiable spectroscopic phase so are listed as ``(unk)'' (i.e., unknown).  Very young SNe II (with very blue featureless continua) similarly have ambiguous phases so are listed as ``(young)''.
}
\end{deluxetable}
\end{landscape}

